Procedural Knowledge Ontology (PKO)

Processes, workflows and guidelines are core to ensure the correct functioning of industrial companies: for the successful operations of factory lines, machinery or services, often industry operators rely on their past experience and know-how. The effect is that this Procedural Knowledge (PK) remains tacit and, as such, difficult to exploit efficiently and effectively. This paper presents PKO, the Procedural Knowledge Ontology, which enables the explicit modeling of procedures and their executions, by reusing and extending existing ontologies. PKO is built on requirements collected from three heterogeneous industrial use cases and can be exploited by any AI and data-driven tools that rely on a shared and interoperable representation to support the governance of PK throughout its life cycle. We describe its structure and design methodology, and outline its relevance, quality, and impact by discussing applications leveraging PKO for PK elicitation and exploitation.

==> LOT.tex <==
% descrizione abbastanza dettagliata di LOT, la metto qui ché potrebbe servire come reference

\paragraph{Ontology requirements specification}
The ontology requirements specification activity refers to the process of defining the goal and scope of the ontology (\emph{Purpose and scope identification} activity) and specifying the requirements that the ontology should satisfy. Such requirements derive from two complementary sub-activities, that is, \emph{Use case specification} and \emph{Data exchange identification}, aiming at collecting the necessary documentation to support knowledge elicitation. During this activity, the collaboration between ontology engineers and domain experts is central.
The output of the use case specification is a list of use cases and user stories that describe different scenarios that need to be supported by the data and modelled within the vocabulary. The output of the data exchange identification is a set of documents and resources (e.g., datasets, standards, data formats, etc.) relevant to the domain to be modeled.
At this point, a \emph{Functional ontological requirements proposal} can be produced, which includes a set of functional requirements in the form of \emph{competency questions} (CQs) and \emph{facts}. 
CQs are questions that the ontology to be developed should answer in order for a user to retrieve relevant information from the data modelled with the ontology \cite{gruninger95cqs}.
Facts are natural language sentences describing the domain modeled by the ontology, possibly including domain-specific terminology (e.g., attributes specifying a certain term to be used in the ontology).
Additionally, a document describing the concepts, the relations, and the relevant attributes of the concepts can be support the translation of competency questions into an ontological model.
Then, in the \emph{Functional ontological requirements completion} activity, domain experts, users and ontology engineers validate whether such requirements are valid and complete. 
All collected and validated requirements should be properly documented (\emph{ORSD formalization}). Optionally, functional requirements can be formalized into test cases (\emph{Functional ontology requirements formalization}).

\paragraph{Ontology implementation}
Before building the ontology using a formal language, an \emph{Ontology conceptualization} is proposed as an initial model informally representing the domain of knowledge, with custom level of detail. Such model usually includes an informal proposal of classes (or concepts), properties between classes (relationships) and between classes and datatypes (attributes), and hierarchies of classes and properties. Then, ontology engineers convert and extend, if needed, the conceptual model in an ontology language such as RDF(S) and OWL, thus performing the \emph{Ontology encoding}. A recommended practice is \emph{Ontology reuse}, i.e., using existing ontological resources that solve the same modelling problems to be addressed, in order to improve interoperability \cite{carriero2020landscape}. Finally, the \emph{Ontology evaluation} activity allows to check the technical quality of an ontology: its coverage of the domain, fit for purpose, inconsistencies, etc.

\paragraph{Ontology publication} 
The aim of this activity is to provide an ontology accessible online, as both a human-readable documentation and a machine-readable file from its URI.
After selecting which ontology version is to be released (\emph{Propose release candidate}), such release needs to be documented with (i) a human-readable description of the ontology and its ontology entities, (ii) relevant metadata (e.g., title, creator, date of creation), (iii) a graphical representation of the ontology, (iv) usage examples to help reuse, (v) the list of requirements addressed. At this point, the ontology can be published online (\emph{Online publication}), following the best practices for vocabularies on the web provided by the W3C\footnote{\url{http://www.w3.org/TR/swbp-vocab-pub/}}, making it accessible via its URI as a file in a formal language and as human-readable documentation using content negotiation.

\paragraph{Ontology maintenance}
The published ontology should be kept available and up-to-date, addressing possible bugs, suggestions, improvements, and new emerging requirements. This activity may also result in the generation of a new ontology version.
